Quantifying OpenMP: Statistical Insights into Usage and Adoption

In high-performance computing (HPC), the demand for efficient parallel programming models has grown dramatically since the end of Dennard Scaling and the subsequent move to multi-core CPUs. OpenMP stands out as a popular choice due to its simplicity and portability, offering a directive-driven approach for shared-memory parallel programming. Despite its wide adoption, however, there is a lack of comprehensive data on the actual usage of OpenMP constructs, hindering unbiased insights into its popularity and evolution. This paper presents a statistical analysis of OpenMP usage and adoption trends based on a novel and extensive database, HPCORPUS, compiled from GitHub repositories containing C, C++, and Fortran code. The results reveal that OpenMP is the dominant parallel programming model, accounting for 45% of all analyzed parallel APIs. Furthermore, it has demonstrated steady and continuous growth in popularity over the past decade. Analyzing specific OpenMP constructs, the study provides in-depth insights into their usage patterns and preferences across the three languages. Notably, we found that while OpenMP has a strong "common core" of constructs in common usage (while the rest of the API is less used), there are new adoption trends as well, such as simd and target directives for accelerated computing and task for irregular parallelism. Overall, this study sheds light on OpenMP's significance in HPC applications and provides valuable data for researchers and practitioners. It showcases OpenMP's versatility, evolving adoption, and relevance in contemporary parallel programming, underlining its continued role in HPC applications and beyond. These statistical insights are essential for making informed decisions about parallelization strategies and provide a foundation for further advancements in parallel programming models and techniques.

==> hpcorpus_apis_dist_hist.tex <==


\begin{figure}[htbp!]
\centering
\begin{tikzpicture}%[scale=0.8]
\begin{axis}  
[  
    ybar,  
    ymax=6500,
    enlargelimits=0.15,  
        ylabel={\# Repositories},
    %xlabel={\ Parallel API},  
    symbolic x coords={
    OpenMP,
    MPI,
    OpenCL,
    CUDA,
    TBB,
    Cilk,
    OpenACC,
    SYCL}, % these are the specification of coordinates on the x-axis.  
    xtick=data,  
        nodes near coords,
        every node near coord/.append style={rotate=90, anchor=west},
    xticklabel style={rotate=50}
    ]  
\addplot coordinates {(OpenMP, 5818) (MPI, 3125) (CUDA, 1360) (OpenCL, 1445) (OpenACC, 101) (SYCL, 34) (TBB, 592) (Cilk, 152) }; 
\end{axis}  
\end{tikzpicture}  
\caption{Parallel API distribution in \hpcorpus{}.
}
\label{fig:histogram_hpcorpus}
\end{figure}


==> hpcorpus_apis_dist_pie.tex <==
\begin{figure}[ht]
\centering
\begin{tikzpicture}[scale=0.650]
\centering
\pie[color={archtOrange,archtBlue,archtRed,mGreen,archtPurple,archtGray,mLightGreen,mLightYellow}]{
    46.0/OpenMP,
    24.7/MPI,
    11.4/OpenCL,
    10.7/CUDA,
    7.2/Others}
\end{tikzpicture}
\caption{Usage of parallel APIs in \hpcorpus{}.} 
\label{fig:pie_chart_hpcorpus}
\end{figure}

==> misc.tex <==
% \begin{itemize} [wide, labelwidth=!, labelindent=0pt]
% \item \textbf{\textit{for} loops: }\textit{for} loops emerge as a vital component, with large occurrence counts.
% In particular, C boasts 21,822,609 occurrences, followed by C++ with 19,841,237, and Fortran with 1,203,773 (do loops).
% These numbers underscore the widespread utilization of \textit{for} loops (or their equivalents in Fortran, \textit{do}) in these languages, highlighting their significance in iterative processes (including \textit{parallel for}).
% While this is also reflected in the number of OpenMPs \textit{for} sections, the proportions are not the same: C has roughly 10\% more \textit{for} loops than C++, but the appearance of OpenMP \textit{for} sections in C++ is more than double compared to C.
% However, proportionally to the amount of \textit{for} loops, Fortran leads with about 1.4\% of all loops being paralleled with OpenMP (compared with C++'s 0.4\% and C's 0.13\%).


% \item \textbf{Scheduling: }The distribution of explicit scheduling methods (\autoref{fig:histogram_scheduling})\footnote{See code @ \href{https://github.com/Scientific-Computing-Lab-NRCN/HPCorpus/blob/121b0f088f3187cf82a54016e82992400cfcfe2c/generate_stats.py\#L255}{get\_scheduling}.} reveals a clear preference for static scheduling across all three languages. Static scheduling stands out as the favored choice, with C exhibiting 8,705 occurrences, followed by C++ with 4,897, and Fortran with 2,013. Although dynamic scheduling shows less prevalence than static scheduling, it still maintains noteworthy usage in comparison to the more sophisticated methods (such as \textit{guided}, \textit{runtime} and \textit{auto}, which are less common.

% \item \textbf{Data-sharing: }The constructs that are responsible for managing data sharing and dependencies, namely \textit{private}, \textit{firstprivate}, \textit{lastprivate}, \textit{shared}, and \textit{reduction}, display varying counts across the languages. Notably, C++ demonstrates higher counts in most cases compared to C and Fortran, indicating its popularity in parallel programming scenarios. Conversely, the \textit{nowait} construct, aimed at eliminating implicit synchronization barriers, exhibits relatively lower counts across all languages.

% \item \textbf{Irregular Parallelism: }The \textit{task} construct, utilized for creating and scheduling independent tasks, shows moderate prevalence across the languages. C displays 1903 occurrences, C++ exhibits 4,169 and Fortran demonstrates 663 occurrences. Similarly, the \textit{sections} construct, employed for dividing work among parallel sections, follows a similar pattern, with C having 1,087 occurrences, C++ having 7,038 occurrences, and Fortran having 387 occurrences.
        
% \item \textbf{Vectorization: } To enable vectorization, one uses the \textit{simd} directive along with appropriate compiler flags. Usage of the \textit{simd} directive is sharply different based on the language: in C++, 54,557 usages were found, while in C and Fortran, there were only 9,942 and 1,199 respectively.

% \item \textbf{Offloading: }The usage of the \textit{target} construct, facilitating the offloading of computations to accelerators such as GPUs, stands out prominently in C++, with an impressive count of 78,9306 occurrences. C and Fortran show 6,199 and 2,532 occurrences, respectively.

% \item \textbf{Synchronization: } The \textit{barrier} construct, used for synchronization and ensuring thread convergence, exhibits varying usage across the languages. C, C++, and Fortran show 2,825, 2,728, and 858 occurrences, respectively. The \textit{atomic} construct, enabling atomic operations on variables in parallel regions, is moderately used, with C, C++, and Fortran exhibiting counts of 3,601, 5,360 and 2,005 occurrences, respectively. In contrast, the \textit{flush} construct, which supports memory consistency among threads, demonstrates relatively lower counts across all three languages, with C, C++, and Fortran recording occurrences of 589, 1,355, and 205, respectively. The \textit{single} construct, specifying regions of code to be executed by a single thread, shows moderate usage. C, C++, and Fortran display counts of 1,019, 3,460, and 533 occurrences, respectively. Notably, the \textit{master} construct, designating a specific thread as the master thread in a parallel region, emerges as relatively common in C++ with 7,732 occurrences, while C and Fortran exhibit counts of 1,244 and 556 occurrences, respectively.
% \end{itemize}


%Since the end of Dennard scaling, multi-core and many-core architectures have gained popularity and are nowadays regarded ubiquitous. The primary method to exploit the potential of these architectures in code parallelization is to use OpenMP, which is an API that supports shared-memory parallelization using compiler directives (pragmas). Over the last decade, OpenMP increasingly gained popularity among programmers and large companies. This growing trend in the use of OpenMP allows us to gather data that can be used for OpenMP-driven research.

% Therefore, we introduce the HPCorpus database, generated by the tool \textit{OpenMP-Extractor}~\footnote{\href{https://github.com/talkad/OpenMPdb}{https://github.com/talkad/OpenMPdb}}.
% Since the for-loop is the most computation intensive component in the code (Hotspot), the database contains for-loops and their corresponding OpenMP directives, if they exist. For-loops with OpenMP directives are tagged with positive labels, whereas the for-loops without OpenMP directives are tagged with negative labels. 





% \section{Insights}
% \begin{enumerate}

% \item OpenMP, as a whole, is getting more and more widespread every year.

% \item Major companies widely accept it in real production applications.

% \item Language Preference: While OpenMP supports Fortran, its predominant usage is in C and C++.

% \item Core Usage Patterns: OpenMP usage focuses on the loop work-sharing construct, indicating a prevalent usage pattern.

% \item Scheduling Methods: Static scheduling is predominantly used, with occasional use of dynamic scheduling, while other methods are less commonly employed.

% \item Thread Synchronization: Thread synchronization is frequently used, implying that users often need to intervene in the code for synchronization purposes.

% \item Code Block Length: Most OpenMP usages involve structured code blocks of up to 50 lines, suggesting a preference for parallelizing smaller sections of code.

% \item Version Adoption: Despite the availability of newer OpenMP versions, the majority of usage remains within OpenMP v4, which was released about a decade ago.

% \item Non-Uniform Feature Adoption: The adoption of new features from each OpenMP version is not uniform, indicating selective adoption of specific features based on user needs.

% \item MPI Usage and Hybrid Paradigms: MPI (Message Passing Interface) is more widely used compared to OpenMP, and hybrid paradigms like MPI+OpenMP are valuable for projects with scalability issues beyond multiple nodes.

% \item OpenMP for GPUs: While CUDA and OpenCL are more commonly used for GPUs, OpenMP for GPUs is gaining momentum.

% \end{enumerate}


% \begin{figure}[!h]
%     \centering
%         \begin{tabular}{|c |c |c |c |} 
%          \hline
%          Description & C & C++ & Fortran  \\ [0.5ex] 
%          \hline\hline
%          \textit{for/do} loops & 21,936,098 & 19,868,390 & 1,203,913 \\
%          \hline
%     \end{tabular}
%     \caption{Total amount of \textit{for/do} loops in HPCorpus.}
% \end{figure}


% \begin{figure}[!h]
%     \centering
%         \begin{tabular}{|c |c |c |c |} 
%          \hline
%          Description & C & C++ & Fortran  \\ [0.5ex] 
%          \hline\hline
%          \textit{for} & 30,185 & 89,726 & 17,660 \\
%          \hline
%          \textit{parallel for} & 22,201 & 71,428 & 7,949 \\
%          \hline
%          \textit{simd} & 9,877 & 54,557 & 1,252 \\
%          \hline
%          \textit{schedule static} & 6,168 & 5,628 & 2,164 \\
%          \hline
%          \textit{schedule dynamic} & 2,093 & 3,823 & 806 \\
%          \hline
%          \textit{private} & 12,885 & 34,412 & 16,660 \\
%          \hline
%          \textit{firstprivate} & 1,908 & 10,363 & 1,559 \\
%          \hline
%          \textit{lastprivate} & 1,623 & 8,519 & 481\\
%          \hline
%          \textit{shared} & 7,712 & 10,194 & 6,016\\
%          \hline
%          \textit{reduction} & 3,056 & 22,875 & 2,819\\
%          \hline
%          \textit{nowait} & 1,008 & 2,274 & 12\\ 
%           \hline
%          \textit{target} & 6,248 & 79,076 & 2,586 \\
%          \hline
%          \textit{task} & 4,501 & 18,270 & 1,695 \\ 
%          \hline
%          \textit{section} & 2,501 & 9,654 & 979 \\ 
%          \hline
%          \textit{critical} & 4,757 & 8,657 & 1,067 \\ 
%          \hline
%          \textit{barrier} & 2,833 & 2,728 & 859\\  
%          \hline
%          \textit{atomic} & 3,652 & 5,394 & 2,085\\ 
%          \hline
%          \textit{flush} & 599 & 1,398 & 205\\ 
%          \hline
%          \textit{single} & 1,027 & 3,469 & 584\\ 
%          \hline
%          \textit{master} & 1,289 & 7,871 & 579\\ 
%          \hline
%     \end{tabular}
%     \caption{HPCorpus OpenMP common directives breakdown.}
% \end{figure}



 
% \begin{figure*}
%   \centering
%   % Version 3
%   \begin{subfigure}{\textwidth}
%     \begin{tikzpicture}
%       \begin{axis}[
%         ybar,
%         width=\textwidth,
%         height=4cm,
%         ylabel={Frequency (ver. 3)},
%         xtick=data,
%         xticklabel style={rotate=30},
%         xticklabels={{task}, {collapse}, {taskwait}, {atomic\_read}, {atomic\_write}, {atomic\_update}, {atomic\_capture}, {task\_final}, {schedule(auto)}, {taskyield}},
%         ymode=log,
%         ymin=1,
%         %ymax=10000,
%         log basis y=10,
%         bar width=4pt,
%         ]

%         % Version 3
%         \addplot coordinates {
%           (1, 4947)
%           (2, 1268)
%           (3, 802)
%           (4, 621)
%           (5, 634)
%           (6, 375)
%           (7, 1152)
%           (8, 46)
%           (9, 39)
%           (10, 39)
%         };
%         \addplot coordinates {
%           (1, 4025)
%           (2, 1656)
%           (3, 665)
%           (4, 180)
%           (5, 212)
%           (6, 397)
%           (7, 1132)
%           (8, 102)
%           (9, 83)
%           (10, 539)
%         };
%         \addplot coordinates {
%           (1, 1870)
%           (2, 4687)
%           (3, 311)
%           (4, 236)
%           (5, 249)
%           (6, 190)
%           (7, 176)
%           (8, 16)
%           (9, 15)
%           (10, 11)
%         };
%       \end{axis}
%     \end{tikzpicture}
%   \end{subfigure}

%   % Version 4
%   \begin{subfigure}{\textwidth}
%     \begin{tikzpicture}
%       \begin{axis}[
%         ybar,
%         width=\textwidth,
%         height=4cm,
%         ylabel={Frequency (ver. 4)},
%         xtick=data,
%         xticklabel style={rotate=30},
%         xticklabels={{simd}, {task\_depend}, {target}, {proc\_bind}, {taskgroup}, {cancel}},
%         ymode=log,
%         ymin=1,
%         %ymax=15000,
%         log basis y=10,
%         bar width=4pt,
%         ]
%         % Version 4
%         \addplot coordinates {
%           (1, 10268)
%           (2, 479)
%           (3, 10459)
%           (4, 259)
%           (5, 627)
%           (6, 2070)
%         };
%         \addplot coordinates {
%           (1, 32706)
%           (2, 240)
%           (3, 49914)
%           (4, 546)
%           (5, 240)
%           (6, 699)
%         };
%         \addplot coordinates {
%           (1, 988)
%           (2, 355)
%           (3, 3789)
%           (4, 71)
%           (5, 327)
%           (6, 461)
%         };
%       \end{axis}
%     \end{tikzpicture}
%   \end{subfigure}

%   % Version 4.5
%   \begin{subfigure}{\textwidth}
%     \begin{tikzpicture}
%       \begin{axis}[
%         ybar,
%         width=\textwidth,
%         height=4cm,
%         ylabel={Frequency (ver. 4.5)},
%         xtick=data,
%         xticklabel style={rotate=30},
%         xticklabels={{target\_private}, {target\_firstprivate}, {simdlen}, {task\_priority}, {linear}, {target\_defaultmap}, {target\_is\_device\_ptr}, {target\_nowait}, {target\_depend}},
%         ymode=log,
%         ymin=1,
%         %ymax=15000,
%         log basis y=10,
%         bar width=4pt,
%         ]
%         % Version 4.5
%         \addplot coordinates {
%           (1, 1233)
%           (2, 463)
%           (3, 1146)
%           (4, 47)
%           (5, 1250)
%           (6, 112)
%           (7, 96)
%           (8, 157)
%           (9, 86)
%         };
%         \addplot coordinates {
%           (1, 4883)
%           (2, 1830)
%           (3, 691)
%           (4, 66)
%           (5, 2864)
%           (6, 1113)
%           (7, 1811)
%           (8, 470)
%           (9, 2883)
%         };
%         \addplot coordinates {
%           (1, 85)
%           (2, 43)
%           (3, 88)
%           (4, 9)
%           (5, 442)
%           (6, 153)
%           (7, 37)
%           (8, 36)
%           (9, 20)
%         };
%       \end{axis}
%     \end{tikzpicture}
%   \end{subfigure}

%   % Version 5
%   \begin{subfigure}{\textwidth}
%     \begin{tikzpicture}
%       \begin{axis}[
%         ybar,
%         width=\textwidth,
%         height=4cm,
%         legend style={at={(0.5,-1)},anchor=north,legend columns=-1},
%         ylabel={Frequency (ver. 5)},
%         xtick=data,
%         xticklabel style={rotate=30},
%         xticklabels={{loop}, {taskloop}, {mutexinoutset}, {requires}, {scan}, {task\_in\_reduction}, {atomic\_hint}, {inscan}, {order(concurrent)}, {taskwait\_depend}, {task\_detach}, {task\_affinity}},
%         ymode=log,
%         ymin=1,
%         %ymax=30000,
%         log basis y=10,
%         bar width=4pt,
%         ]
%         % Version 5
%         \addplot coordinates {
%           (1, 26954)
%           (2, 1903)
%           (3, 26)
%           (4, 258)
%           (5, 1517)
%           (6, 121)
%           (7, 48)
%           (8, 175)
%           (9, 138)
%           (10, 24)
%           (11, 42)
%           (12, 158)
%         };
%         \addplot coordinates {
%           (1, 10495)
%           (2, 8619)
%           (3, 336)
%           (4, 1092)
%           (5, 1226)
%           (6, 1130)
%           (7, 13)
%           (8, 56)
%           (9, 38)
%           (10, 36)
%           (11, 52)
%           (12, 96)
%         };
%         \addplot coordinates {
%           (1, 688)
%           (2, 432)
%           (3, 24)
%           (4, 113)
%           (5, 128)
%           (6, 33)
%           (7, 76)
%           (8, 84)
%           (9, 129)
%           (10, 21)
%           (11, 39)
%           (12, 39)
%         };

%         \legend{C, C++, Fortran}
%       \end{axis}
%     \end{tikzpicture}
    
%     % \caption*{OpenMP clauses and functions}
%     \label{fig:version5}
%   \end{subfigure}

%   \caption{Distribution of OpenMP clauses over different versions.}
% \end{figure*}



% \begin{figure*}
%   \centering
%   % Version 3
%   \begin{subfigure}{\textwidth}
%     \begin{tikzpicture}
%       \begin{axis}[
%         ybar,
%         width=\textwidth,
%         height=4cm,
%         ylabel={Frequency (ver. 3)},
%         xtick=data,
%         xticklabel style={rotate=30},
%         xticklabels={{task}, {collapse}, {taskwait}, {atomic\_capture}, {atomic\_update}, {schedule(auto)}, {atomic\_write}, {atomic\_read}, {taskyield}, {task\_mergeable}, {task\_final}},
%         ymode=log,
%         ymin=1,
%         ymax=10000,
%         log basis y=10,
%         ]
%         % Version 3

%       \end{axis}
%     \end{tikzpicture}
%   \end{subfigure}

%   % Version 4
%   \begin{subfigure}{\textwidth}
%     \begin{tikzpicture}
%       \begin{axis}[
%         ybar,
%         width=\textwidth,
%         height=4cm,
%         ylabel={Frequency (ver. 4)},
%         xtick=data,
%         xticklabel style={rotate=30},
%         xticklabels={{simd}, {target}, {taskgroup}, {proc\_bind}, {cancel}, {task\_depend}},
%         ymode=log,
%         ymin=1,
%         ymax=15000,
%         log basis y=10,
%         ]
%         % Version 4
%         \addplot coordinates {
%           (1, 32706)
%           (2, 49914)
%           (3, 901)
%           (4, 546)
%           (5, 699)
%           (6, 240)
%         };
%       \end{axis}
%     \end{tikzpicture}
%   \end{subfigure}

%   % Version 4.5
%   \begin{subfigure}{\textwidth}
%     \begin{tikzpicture}
%       \begin{axis}[
%         ybar,
%         width=\textwidth,
%         height=4cm,
%         ylabel={Frequency (ver. 4.5)},
%         xtick=data,
%         xticklabel style={rotate=30},
%         xticklabels={{target\_private}, {target\_is\_device\_ptr}, {target\_firstprivate}, {linear}, {target\_nowait}, {target\_depend}, {target\_defaultmap}, {simdlen}, {task\_priority}},
%         ymode=log,
%         ymin=1,
%         ymax=15000,
%         log basis y=10,
%         ]
%         % Version 4.5
%         \addplot coordinates {
%           (1, 4883)
%           (2, 1811)
%           (3, 1830)
%           (4, 2864)
%           (5, 470)
%           (6, 2883)
%           (7, 1113)
%           (8, 691)
%           (9, 66)
%         };
%       \end{axis}
%     \end{tikzpicture}
%   \end{subfigure}

%   % Version 5
%   \begin{subfigure}{\textwidth}
%     \begin{tikzpicture}
%       \begin{axis}[
%         ybar,
%         width=\textwidth,
%         height=4cm,
%         ylabel={Frequency (ver. 5)},
%         xtick=data,
%         xticklabel style={rotate=30},
%         xticklabels={{loop}, {taskloop}, {scan}, {requires}, {task\_in\_reduction}, {order(concurrent)}, {mutexinoutset}, {inscan}, {taskwait\_depend}, {atomic\_hint}, {task\_affinity}, {task\_detach}},
%         ymode=log,
%         ymin=1,
%         ymax=30000,
%         log basis y=10,
%         ]
%         % Version 5
%         \addplot coordinates {
%           (1, 10495)
%           (2, 8619)
%           (3, 1226)
%           (4, 1092)
%           (5, 1130)
%           (6, 38)
%           (7, 336)
%           (8, 56)
%           (9, 36)
%           (10, 13)
%           (11, 96)
%           (12, 52)
%         };
%       \end{axis}
%     \end{tikzpicture}
%     \caption*{OpenMP clauses and functions}
%     \label{fig:version5}
%   \end{subfigure}
%   \caption{Distribution of OpenMP clauses over different versions for C++ codes. Version 2 includes 449,197 clauses.}
% \end{figure*}





% \begin{figure*}
%   % Version 3
%   \begin{subfigure}{\textwidth}
%     \begin{tikzpicture}
%       \begin{axis}[
%         ybar,
%         width=\textwidth,
%         height=4cm,
%         ylabel={Frequency (ver. 3)},
%         xtick=data,
%         xticklabel style={rotate=30},
%         xticklabels={{task}, {taskwait}, {collapse}, {atomic\_write}, {atomic\_read}, {atomic\_capture}, {atomic\_update}, {task\_final}, {taskyield}, {schedule(auto)}},
%         ymode=log,
%         ymin=1,
%         ymax=10000,
%         log basis y=10,
%         ]
%         % Version 3
%         \addplot coordinates {
%           (1, 1870)
%           (2, 311)
%           (3, 4687)
%           (4, 249)
%           (5, 236)
%           (6, 176)
%           (7, 190)
%           (8, 16)
%           (9, 11)
%           (10, 15)
%         };
%       \end{axis}
%     \end{tikzpicture}
%   \end{subfigure}

%   % Version 4
%   \begin{subfigure}{\textwidth}
%     \begin{tikzpicture}
%       \begin{axis}[
%         ybar,
%         width=\textwidth,
%         height=4cm,
%         ylabel={Frequency (ver. 4)},
%         xtick=data,
%         xticklabel style={rotate=30},
%         xticklabels={{target}, {simd}, {task\_depend}, {taskgroup}, {cancel}, {proc\_bind}},
%         ymode=log,
%         ymin=1,
%         ymax=15000,
%         log basis y=10,
%         ]
%         % Version 4
%         \addplot coordinates {
%           (1, 3789)
%           (2, 988)
%           (3, 355)
%           (4, 327)
%           (5, 461)
%           (6, 71)
%         };
%       \end{axis}
%     \end{tikzpicture}
%   \end{subfigure}

%   % Version 4.5
%   \begin{subfigure}{\textwidth}
%     \begin{tikzpicture}
%       \begin{axis}[
%         ybar,
%         width=\textwidth,
%         height=4cm,
%         ylabel={Frequency (ver. 4.5)},
%         xtick=data,
%         xticklabel style={rotate=30},
%         xticklabels={{linear}, {target\_defaultmap}, {target\_nowait}, {target\_private}, {simdlen}, {task\_priority}, {target\_firstprivate}, {target\_depend}, {target\_is\_device\_ptr}},
%         ymode=log,
%         ymin=1,
%         ymax=15000,
%         log basis y=10,
%         ]
%         % Version 4.5
%         \addplot coordinates {
%           (1, 442)
%           (2, 153)
%           (3, 36)
%           (4, 85)
%           (5, 88)
%           (6, 9)
%           (7, 43)
%           (8, 20)
%           (9, 37)
%         };
%       \end{axis}
%     \end{tikzpicture}
%   \end{subfigure}

%   % Version 5
%   \begin{subfigure}{\textwidth}
%     \begin{tikzpicture}
%       \begin{axis}[
%         ybar,
%         width=\textwidth,
%         height=4cm,
%         ylabel={Frequency (ver. 5)},
%         xtick=data,
%         xticklabel style={rotate=30},
%         xticklabels={{loop}, {taskloop}, {task\_affinity}, {requires}, {task\_detach}, {atomic\_hint}, {task\_in\_reduction}, {taskwait\_depend}, {mutexinoutset}, {scan}, {inscan}, {order(concurrent)}},
%         ymode=log,
%         ymin=1,
%         ymax=30000,
%         log basis y=10,
%         ]
%         % Version 5
%         \addplot coordinates {
%           (1, 688)
%           (2, 432)
%           (3, 39)
%           (4, 113)
%           (5, 39)
%           (6, 76)
%           (7, 33)
%           (8, 21)
%           (9, 24)
%           (10, 128)
%           (11, 84)
%           (12, 129)
%         };
%       \end{axis}
%     \end{tikzpicture}
%     \caption*{OpenMP clauses and functions}
%     \label{fig:version5}
%   \end{subfigure}
%   \caption{Distribution of OpenMP clauses over different versions for Fortran codes. Version 2 includes 57,828 clauses.}
% \end{figure*}



